Relevance-guided Unsupervised Discovery of Abilities with Quality-Diversity Algorithms

Quality-Diversity algorithms provide efficient mechanisms to generate large collections of diverse and high-performing solutions, which have shown to be instrumental for solving downstream tasks. However, most of those algorithms rely on a behavioural descriptor to characterise the diversity that is hand-coded, hence requiring prior knowledge about the considered tasks. In this work, we introduce Relevance-guided Unsupervised Discovery of Abilities; a Quality-Diversity algorithm that autonomously finds a behavioural characterisation tailored to the task at hand. In particular, our method introduces a custom diversity metric that leads to higher densities of solutions near the areas of interest in the learnt behavioural descriptor space. We evaluate our approach on a simulated robotic environment, where the robot has to autonomously discover its abilities based on its full sensory data. We evaluated the algorithms on three tasks: navigation to random targets, moving forward with a high velocity, and performing half-rolls. The experimental results show that our method manages to discover collections of solutions that are not only diverse, but also well-adapted to the considered downstream task.

==> algorithms/aurora.tex <==
\begin{algorithm}[t]
  \small
  \caption{\aurora{} (number of iterations $I$; encoder $\encoder$; target container size $\targetscC$, container update period $T_\cC$)}
  \label{algo:aurora}
  
  \newcommand\algorithmicitemindent{\hspace*{\algorithmicindent}\hspace*{\algorithmicindent}}
  

  \begin{algorithmic}[1]
    \State{$\metrics \gets \text{Euclidiean distance}$}
    \State{$\container \gets \emptyset$}

    \State{Initialise $\thresholdNov$}
    \For{$iter$ = 1 $\rightarrow I$}
    
    \State{$\container \gets$ \Call{QD\_Iteration}{$iter$, $\container$, $\encoder$, $\metrics$}}
    
    \If{encoder update expected at iteration $iter$} 
        \State{$\{\encoder, \container\} \gets$ \Call{Encoder\_Update}{$\encoder$, $\container$}}
    \EndIf
    \State{$\{\container, \thresholdNov\} \gets$ \Call{Manage\_Container\_Size}{$\container, \thresholdNov, \targetscC, T_\cC$}}

      \EndFor\label{auroraendfor}
      \State{\Return container $\container$}
      
\item[]
    \Procedure{QD\_Iteration}{$iter$, $\container$, $\encoder$, $\metrics$}
          \If{first iteration}
      \State{$\vect{pop_{parents}} \gets $ random()}
      \State{$\vect{pop_{offspring}} \gets $ random()}
    \Else
        \State{$\vect{pop_{parents}} \gets $ selection($\container$) }
        \State{$\vect{pop_{offspring}} \gets $ random\_variation($\vect{pop_{parents}}$) }
    \EndIf
    \ForEach{$indiv$ in $\vect{pop_{offspring}}$}
    \State{$\{\obsindiv,  \perfindiv\}  \gets$ evaluate($indiv$) }
    \State{$\bdpropindiv \gets\encoder(\obsindiv)$} 
    \State{$\container \gets$ attempt\_add\_to\_container($indiv$, $\container$, $\metrics$)} 
    \EndFor
    
    \State{\Return $\container$}
    \EndProcedure
 
\item[]
   
    \Procedure{Encoder\_Update}{$\container$, $\encoder$}
        \State{$\encoder \gets$ train($\encoder$, $\container$)}
        \State{$\container \gets$ update\_descriptors\_in\_container($\container$, $\encoder$)} 
        \State{\Return $\encoder, \container$}
    \EndProcedure
    
\item[]

    \Procedure{Manage\_Container\_Size}{$\container, \thresholdNov, \targetscC, T_\cC$}
          \State{$\thresholdNov \gets$ update\_threshold\_distance($\thresholdNov$, $\scC$, $\targetscC$) }\label{algo:aurora:update_threshold}
        \If{$iter$ multiple of $T_\cC$} 
            \State{$\container \gets$ update\_container($\container$, $\thresholdNov$)}  \label{algo:aurora:update_container}  %TODO: Provide more insights on the role played by this part. 
        \EndIf
        
        \State{\Return $\container, \thresholdNov$}
    \EndProcedure
     
  \end{algorithmic}
\end{algorithm}




==> tables/hyperparameters.tex <==
\begin{table}[t]
    \centering
    % \small


    \begin{threeparttable}
    \begin{tabular}{l l}
    \toprule
    Hyperparameter & Value \\
        \midrule
    	\addlinespace
    Hyperparameter & Value \\

    \bottomrule
    	
    \end{tabular}
    
    % \begin{tablenotes}
    %      \item[1] CSC and VAT correspond respectively to the \textit{Container Size Control} and the \textit{Volume Adaptive Threshold} techniques. 
    %      \item[2] HC refers to \textit{Hand-Coded}.
    %  \end{tablenotes}
    \end{threeparttable}

\caption[Hyperparameters]{
    Hyperparameters
    }
    \label{table:variants}

\end{table}

